Assessing the Robustness of Bayesian Dark Knowledge to Posterior Uncertainty

Bayesian Dark Knowledge is a method for compressing the posterior predictive distribution of a neural network model into a more compact form. Specifically, the method attempts to compress a Monte Carlo approximation to the parameter posterior into a single network representing the posterior predictive distribution. Further, the authors show that this approach is successful in the classification setting using a student network whose architecture matches that of a single network in the teacher ensemble. In this work, we examine the robustness of Bayesian Dark Knowledge to higher levels of posterior uncertainty. We show that using a student network that matches the teacher architecture may fail to yield acceptable performance. We study an approach to close the resulting performance gap by increasing student model capacity.

==> archived_sections/intro_v1.tex <==
\section{Introduction}

Deep learning models have shown promising results in the areas of computer vision, natural language processing and speech recognition, surpassing the performance of its counterparts as well as human-level \cite{graves2013hybrid, graves2013speech, krizhevsky2012imagenet}. However, the efficacy of such models is largely dependent of vast amounts of labeled data. Neural networks are also known to produce over-confident results (sometimes, even without adverserial inputs) which can be dangerous in more serious applications like medical imaging, self-driving cars, etc. Among all the techniques to overcome these challenges, we turn our focus to Bayesian Inference. In Bayesian Inference, we utilize the Bayes theorem to obtain the posterior distribution over the parameters of our given model. For a given model, let the parameter set be denoted as  $\theta$, and the training set $\pazocal{D} = \{(\mathbf{x_i}, y_{i})\}_{i=1} ^ N$, where each $\mathbf{x}_i$ denotes a $d$-dimensional feature input corresponding to the input indexed at $i$ and $y_i$ denotes an integer for a classification problem or a continuous real value for a regression problem. The prior distribution over the parameter set is denoted as $p(\theta)$. Thus, we obtain the posterior distribution as 
\begin{equation}
    \label{eq:posterior}
    p(\theta|\pazocal{D}) = \frac{p(\pazocal{D}|\theta)p(\theta)}{\int p(\pazocal{D}|\theta)p(\theta) d\theta}
\end{equation}
Ultimately, we obtain the posterior predictive distribution as following:
\begin{equation}
\label{eq:posterior_predictive}
p(y| \mathbf{x}, \pazocal{D}) = \int p(y|\mathbf{x}, \theta) p(\theta|\pazocal{D}) d\theta
\end{equation}
The challenging part in the process of obtaining a posterior predictive distribution is that the integral term (also known as evidence) in equation \ref{eq:posterior} is not always analytically tractable. There are existing methods in the area of variational learning and markov chain monte carlo (MCMC) based sampling techniques to circumvent this challenge. In this study, we focus on a technique that stems out of the combination of an MCMC based sampling technique and knowledge distillation for neural networks \cite{balan2015bayesian, welling2011bayesian, hinton2015distilling}. This technique aims to produce a posterior predictive distribution using a single neural network model of the same size and architecture as the model of our choice, trained using multiple parameter samples from the approximate posterior distribution. We employ this method to the task of classifying where a portion of the pixels have been masked out.  Another way to interpret this task is to think of it as classifying images under occlusion or classifying data points with missing values. Since both these applications are of particular use in practical scenarios, it becomes all the more important to analyze the performance of this method on tasks like these. As we see in the experimental sections of the paper, knowledge distillation into a model of same size, doesn't lead to the same level of performance as the monte carlo estimate of equation \ref{eq:posterior_predictive} obtained using all the samples generated from the approximate posterior distribution. Finally, as an attempt to mitigate this gap, we suggest that increasing the model capacity can further lead to a decrease in the performance gap. We verify this proposition using additional experiments. 


==> archived_sections/related_work_v1.tex <==
\section{Related Work}
In cases where the posterior distribution is not analytically tractable, we try to approximate it. Of all the techniques present in the literature for bayesian neural networks, variational inference (VI) and MCMC based sampling methods have been more popular than the rest \cite{jordan1999introduction, Neal:1996:BLN:525544, welling2011bayesian}. In VI, we define an auxiliary distribution of our choice $q_{\phi} (\theta)$, parameterised by $\phi$ to approximate the true posterior $p(\theta | \pazocal{D})$. The reason for doing this is to get an approximation which can be plugged in the place of $p(\theta | \pazocal{D})$ in equation \ref{eq:posterior_predictive}. Next, we optimize the Kullback-Leibler (KL) divergence between $q_{\phi} (\theta)$ and $p(\theta | \pazocal{D})$:
\begin{equation}
\textrm{KL}(q_{\phi} (\theta) || p(\theta | \pazocal{D})) = \int q_{\phi}(\theta) \log \frac{q_{\phi}(\theta)}{p(\theta | \pazocal{D})}
\end{equation}
Upon further simplification, we obtain that minimizing the KL divergence is equivalent to maximising the following objective:
\begin{equation}
\pazocal{L(\phi)} = \int q_{\phi}(\theta) \log p(\pazocal{D}| \theta) d\theta - \textrm{KL} (q_{\phi}(\theta) || p(\theta))
\end{equation}
This is also known as the evidence lower bound (ELBO) loss. For tractable integral in the first term of our ELBO term, we would typically want a simpler distribution parameterised in $\phi$. However, a simpler distribution doesn't align well with the true posterior and thus, this creates a trade-off between the expressive power of $q_{\phi}(\theta)$ and ease of computation. Another closely related technique is expectation propogation (EP) \cite{minka2001expectation}. The main difference between VI and EP is that in VI, we minimize the $\textrm{KL}(q_{\phi} (\theta) || p(\theta | \pazocal{D}))$, while in EP we minimize $\textrm{KL}(p(\theta | \pazocal{D}) || q_{\phi} (\theta))$. While these methods are useful to obtain an approximate parameterised posterior distribution, they present some challenges when employed in their conventional form. First, the computation cost scales with the amount of data. Secondly, variational methods have a mode-seeking behaviour and this can also lead to a poor approximation of the distribution. A more recent approach has been proposed to tackle the second problem which is known as probabilistic backpropagation (PBP). PBP assumes an already factorised structure for the posterior distribution suitable for tractability in equation \ref{eq:posterior_predictive} and then directly optimizes the posterior predictive distribution to find the parameters of the factorised distribution \cite{hernandez2015probabilistic}. \\
The other line of work extends on MCMC based sampling techniques. Of all the techniques present in the literature, stochastic gradient langevin dynamics (SGLD) \cite{welling2011bayesian} is of primary interest to our study. \emph{Bayesian Dark Knowledge} uses SGLD  to sample from the approximate posterior distribution to train a teacher neural network. Next, we aim to train a student neural network which approximates the bayesian predictive distribution of the teacher neural network. Before we outline the method proposed in, we establish some more notation. Let $p(\theta| \lambda)$ define the prior distribution over the teacher's model parameters $\theta$, parameterised by $\lambda$. In this case, the prior distribution is spherical gaussian distribution centered at $0$ and having precision as $\lambda$. We define the softmax outputs from teacher model using parameters $\theta$ as $p(y_i|\mathbf{x_i}, \theta)$. Next, we define $\pazocal{S}$ as a minibatch of size M drawn from $\pazocal{D}$. Let the total number of training samples in $\pazocal{D}$ be denoted as $N$. $\theta_t$ denotes the parameter set sampled for teacher model at sampling iteration $t$, while $\eta_t$ denotes the learning rate for teacher model at iteration $t$. The langevin noise here is denoted as $z_t \sim \pazocal{N}(0, \eta_t I )$.  Thus, the sampling step for SGLD can be written as:
\begin{equation}
\theta_{t+1} = \theta_{t}+\frac{\eta_{t}}{2}\left(\nabla_{\theta} \log p(\theta | \lambda)+\frac{N}{M} \sum_{i \in \pazocal{S}} \nabla_{\theta} \log p\left(y_{i} | x_{i}, \theta_{t}\right)\right)+ z_{t}
\end{equation}
At this point, let us generate another batch of samples $\pazocal{D'}$ which are used to train the student neural network. One way to obtain $\pazocal{D'}$ by adding gaussian noise of small magnitude to $\pazocal{S}$. The samples from $\pazocal{D'}$ are denoted as $\{(\mathbf{x'_{i}}, y'_{i})\}$. The predictive posterior distribution over $\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}$ using teacher model with parameter set $\theta_{t+1}$ is given as $p(y'_i|\mathbf{x'_i}, \theta_{t+1})$. Similarly, the 
predictive distribution for a student model parameterised by $\omega_t$ is given as $S(y'_i|\mathbf{x'_i}, \omega_t)$. We define the cross-entropy loss between predictive distributions of teacher and student at iteration $t+1$ as
\begin{align*}
\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = -\sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}} \sum_{k=1}^{K} p(y'_i = k|\mathbf{x'_i}, \theta_{t+1}) \log S(y'_i = k|\mathbf{x'_i}, \omega_t)
\end{align*}
At this point, we minimize the above loss by making one optimization update to obtain $\omega_{t+1}$. After all the optimization iterations, we utilize the final parameter set obtained for the student model to make predictions. In the experiments performed by \cite{balan2015bayesian}, they utilize the MNIST dataset with fully-observed images. We argue that the task of classifying MNIST images is relatively easy as a fully connected network used by them achieves a log-likelihood of $1.271 \pm 0.0126$ on test set while trained on 50,000 images. Thus, to analyse this method in more detail, we run extensive experiments on MNIST dataset with masked inputs. 

==> archived_sections/related_work_v2.tex <==
\section{Related Work}
In cases where the posterior distribution is not analytically tractable, we try to approximate it. Some of the previous work done in this direction adapts on the line VI and markov chain monte carlo (MCMC) based sampling methods \cite{jordan1999introduction, Neal:1996:BLN:525544, welling2011bayesian}. In VI, we define an auxiliary distribution of our choice $q_{\phi} (\theta)$, parameterised by $\phi$ to approximate the true posterior $p(\theta | \pazocal{D})$. Next, we optimize the Kullback-Leibler (KL) divergence between $q_{\phi} (\theta)$ and $p(\theta | \pazocal{D})$. \cite{hinton1993keeping} presented the first study to apply VI for neural networks. However, the method presented scalability issues, and to tackle those issues, \cite{graves2011practical} presented an approach using stochastic VI. Another related approach to VI is expectation propagation (EP) \cite{minka2001expectation}. The main difference between VI and EP is that in VI, we minimize the $\textrm{KL}(q_{\phi} (\theta) || p(\theta | \pazocal{D}))$, while in EP we minimize $\textrm{KL}(p(\theta | \pazocal{D}) || q_{\phi} (\theta))$. \citet{soudry2014expectation} shows an online EP algorithm for neural networks with the flexibility of continous weights as well as discrete weights. Another related approach is probabilistic backpropagation (PBP) \cite{hernandez2015probabilistic}. In PBP, we define a parameterised distribution over all the layers over neural network and backpropagate by computing the gradient of the marginal log-likelihood  w.r.t. these parameters. A common problem though with EP and PBP is that they use a diagonal gaussian structure for approximating the posterior distribution. This does not model complex relationships between parameters in the model. To tackle this problem, \citet{louizos2017multiplicative} introduced the concept of \emph{Multiplicative Normalizing Flows}. Under \emph{Multiplicative Normalizing Flows}, we apply a chain of transformations to parameters sampled from our approximate posterior $q_{\phi}(\theta)$, using some additional learnable parameters $\omega$. This technique helps us create samples imitating more complex distributions than the standard mean-field inference. However, this requires the flow to be invertible.

The other line of work extends on MCMC based sampling techniques to sample from approximate posterior distribution and get a monte carlo average of equation \ref{eq:posterior_predictive}. One of the earliest studies in this line of work utilizes Hamiltonian Monte Carlo (HMC) \cite{Neal:1996:BLN:525544} for neural networks. The bottleneck with this method is that it utilizes the full dataset for computing the gradient, subjecting it to scalability issues. This issue has been targeted by stochastic gradient based MCMC algorithms like stochastic gradient langevin dynamics (SGLD) \cite{welling2011bayesian}. SGLD can be seen as fusion of the original SGD algorithm and langevin dynamics. Under SGLD, the earlier iterations of training are used to reach a local mode and then the langevin noise is used to sample around the local mode. \emph{Bayesian Dark Knowledge} \cite{balan2015bayesian} uses SGLD  to sample from the approximate posterior distribution to train a teacher neural network. Next, it aims to train a student neural network which approximates the bayesian predictive distribution of the teacher neural network. With the advent of \emph{Generative Adverserial Networks} \cite{goodfellow2014generative}, there has been some effort behind generative processes for posterior sampling. \citet{wang2018adversarial} introduces a method of distilling the posterior distribution to a generative process, which can be trained in an adverserial fashion. \citet{wang2018adversarial} utilizes the samples generated from SGLD to train a generator. Thus, at test time, rather than running SGLD, posterior samples are generated using the GAN. This approach gives flexibility in terms of computational budget while doing bayesian inference. Another related approach is proposed by \citet{henning2018approximating} where they train a hypernetwork using adverserial training regime. Their method varies slightly from that of \citet{wang2018adversarial} in the sense that the discriminator has to differentiate between pairs of the original input and two possible outputs: one obtained via posterior predictive distribution generated using SGLD and another generated using the GAN. A major difference between \emph{Bayesian Dark Knowledge} and GAN based distillation methods is that the latter set of methods still rely on generating samples for at test time, while the former requires just a single forward pass through the student neural network to produce an estimate of $p(y|\mathbf{x}, \pazocal{D})$. And finally, there's some work which doesn't exactly fit as extensions of VI, EP or MCMC based methods \cite{gal2016dropout, lakshminarayanan2017simple}. \citet{gal2016dropout} suggests a method of quantifying uncertainty by using \emph{dropout} \cite{srivastava2014dropout} at the time of test as well. This method has been termed as MC-dropout and it requires multiple forward passed to get uncertainty in the output. \citet{lakshminarayanan2017simple} implements a simple and scalable technique of utilizing an  ensemble of deep neural networks using proper scoring rules. It uses adverserial style of training to smoothen predictive distributions.

Now, we take a closer look at the distillation technique proposed by \citet{balan2015bayesian}. Before we outline the method proposed in, we establish some more notation. Let $p(\theta| \lambda)$ define the prior distribution over the teacher's model parameters $\theta$, parameterised by $\lambda$. In this case, the prior distribution is a spherical gaussian distribution centered at $0$ with precision denoted as $\lambda$. Next, we define $\pazocal{S}$ as a minibatch of size M drawn from $\pazocal{D}$. Let the total number of training samples in $\pazocal{D}$ be denoted as $N$. $\theta_t$ denotes the parameter set sampled for teacher model at sampling iteration $t$, while $\eta_t$ denotes the learning rate for teacher model at iteration $t$. The langevin noise here is denoted as $z_t \sim \pazocal{N}(0, \eta_t I )$.  Thus, the sampling update for SGLD can be written as:
\begin{equation}
\Delta \theta_{t+1} \!=\!\frac{\eta_{t}}{2}\!\left(\!\nabla_{\theta} \log p(\theta | \lambda)\!+\!\frac{N}{M} \sum_{i \in \pazocal{S}} \nabla_{\theta} \log p\left(y_{i} | x_{i}, \theta_{t}\right)\!\right)+ z_{t}.
\end{equation}
At this point, we generate another batch of samples $\pazocal{D'}$ which are used to train the student neural network. $\pazocal{D'}$ is obtained by adding gaussian noise of small magnitude to $\pazocal{S}$. The samples from $\pazocal{D'}$ are denoted as $\{(\mathbf{x'_{i}}, y'_{i})\}$. The predictive distribution over $\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}$ using teacher model with parameter set $\theta_{t+1}$ is given as $p(y'_i|\mathbf{x'}_i, \theta_{t+1})$. Similarly, the 
predictive distribution for a student model parameterised by $\omega_t$ is given as $S(y'_i|\mathbf{x'}_i, \omega_t)$. The objective for student model is  $\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = \sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}}\textrm{KL}(S(y'_i|\mathbf{x'_i}, \omega_t) || p(y'_i|\mathbf{x'}_i, \theta_{t+1}))$ and run a single optimization iteration to obtain $\omega_{t+1}$. We run this process of sequentially obtaining $\theta_{t+1}$ and $\omega_{t+1}$ until we converge. 


% We define the cross-entropy loss between predictive distributions of teacher and student at iteration $t+1$ as
% \begin{align*}
% &\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = \\
% &\quad-\!\!\!\!\!\!\sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}} \sum_{k=1}^{K} p(y'_i = k|\mathbf{x'_i}, \theta_{t+1}) \log S(y'_i = k|\mathbf{x'_i}, \omega_t).
% \end{align*}
% At this point, we minimize the above loss by making one optimization update to obtain $\omega_{t+1}$. After all the optimization iterations, we utilize the final parameter set obtained for the student model to make predictions.

==> cuts.tex <==



The Bayesian Dark Knowledge approach 


However, they pose significant challenges in terms of high training data requirement as well as bring over-confident while making wrong predictions. Bayesian Inference is a fundamental technique to overcome these challenges. In Bayesian Inference, we utilize the Bayes theorem to obtain the posterior distribution over the parameters of our given model. For a given model, let the parameter set be denoted as  $\theta$, and the training set $\pazocal{D} = \{(\mathbf{x}_i, y_{i})\}_{i=1} ^ N$, where each $\mathbf{x}_i \in \mathbb{R}^d$ denotes a $d$-dimensional feature input corresponding to the input indexed at $i$ and $y_i$ denotes an integer for a classification problem or a continuous real value for a regression problem. The prior distribution over the parameter set is denoted as $p(\theta)$. Thus, we obtain the posterior distribution as 
\begin{equation}
    \label{eq:posterior}
    p(\theta|\pazocal{D}) = \frac{p(\pazocal{D}|\theta)p(\theta)}{\int p(\pazocal{D}|\theta)p(\theta) d\theta}
\end{equation}
Ultimately, we obtain the posterior predictive distribution as following:
\begin{equation}
\label{eq:posterior_predictive}
p(y| \mathbf{x}, \pazocal{D}) = \int p(y|\mathbf{x}, \theta) p(\theta|\pazocal{D}) d\theta
\end{equation}
The challenging part here is that the integral term (also known as evidence) in equation \ref{eq:posterior} is not always analytically tractable. There are existing methods to circumvent this problem based on variational inference (VI), markov chain monte carlo (MCMC) methods, and more recently GAN based methods to approximate the posterior distribution. Among all these methods, the focus of our study is \emph{Bayesian Dark Knowledge}. 

A key advantage of \emph{Bayesian Dark Knowledge} over its counterparts is that it performs ``distillation" of the approximate posterior predictive distribution to a single compact model. At the time of testing, it requires only a single forward pass through the trained ``student" model to approximate equation \ref{eq:posterior_predictive}. A useful application of this can be in low-latency embedded systems where we wish to account for uncertainty without having to store parameter samples or performing multiple forward-passes through a model as required by some other techniques. While the idea is promising, the experimental validations by \cite{balan2015bayesian} are not robust. The experimental validations done on fully observed MNIST dataset for the classification problem point to the fact that there is a low posterior uncertainty in the first place, as evident from the high log-likelihood values on the test set.  Thus, the performance of the technique remains untested against other higher levels of posterior uncertainty. We aim to address this issue through our study. The main goal of this paper is to evaluate the method of \emph{Bayesian Dark Knowledge} under different levels of posterior uncertainty. As we see in the later sections of the paper, we find that the original claim made by \citet{balan2015bayesian} of distilling the posterior predictive distribution to a student model of the same size doesn't hold true. We further show that increasing the model capacity can help mitigate this performance gap to some extent.

-----------------

And finally, there's some work which doesn't exactly fit as extensions of VI, EP or MCMC based methods \cite{gal2016dropout, lakshminarayanan2017simple}. \citet{gal2016dropout} suggests a method of quantifying uncertainty by using \emph{dropout} \cite{srivastava2014dropout} at the time of test as well. This method has been termed as MC-dropout and it requires multiple forward passed to get uncertainty in the output. \citet{lakshminarayanan2017simple} implements a simple and scalable technique of utilizing an  ensemble of deep neural networks using proper scoring rules. It uses adverserial style of training to smoothen predictive distributions.

Now, we take a closer look at the distillation technique proposed by 


% We define the cross-entropy loss between predictive distributions of teacher and student at iteration $t+1$ as
% \begin{align*}
% &\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = \\
% &\quad-\!\!\!\!\!\!\sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}} \sum_{k=1}^{K} p(y'_i = k|\mathbf{x'_i}, \theta_{t+1}) \log S(y'_i = k|\mathbf{x'_i}, \omega_t).
% \end{align*}
% At this point, we minimize the above loss by making one optimization update to obtain $\omega_{t+1}$. After all the optimization iterations, we utilize the final parameter set obtained for the student model to make predictions.






introduces a method of distilling the posterior distribution to a generative process, which can be trained in an adverserial fashion. \citet{wang2018adversarial} uses the samples generated from SGLD to train a generator. Thus, at test time, rather than running SGLD, posterior samples are generated using the GAN. 

Another related approach is proposed by \citet{henning2018approximating} where they train a hypernetwork using an adverserial training regime. Their method varies slightly from that of \citet{wang2018adversarial} in the sense that the discriminator has to differentiate between pairs of the original input and two possible outputs: one obtained via posterior predictive distribution generated using SGLD and another generated using the GAN. A major difference between \emph{Bayesian Dark Knowledge} and GAN based distillation methods is that the latter set of methods still rely on generating samples for at test time, while the former requires just a single forward pass through the student neural network to produce an estimate of $p(y|\mathbf{x}, \pazocal{D})$. 
